Standard vs. Modular Sampling: Best Practices for Reliable LLM Unlearning

A conventional LLM Unlearning setting consists of two subsets -"forget" and "retain", with the objectives of removing the undesired knowledge from the forget set while preserving the remaining knowledge from the retain. In privacy-focused unlearning research, a retain set is often further divided into neighbor sets, containing either directly or indirectly connected to the forget targets; and augmented by a general-knowledge set. A common practice in existing benchmarks is to employ only a single neighbor set, with general knowledge which fails to reflect the real-world data complexities and relationships. LLM Unlearning typically involves 1:1 sampling or cyclic iteration sampling. However, the efficacy and stability of these de facto standards have not been critically examined. In this study, we systematically evaluate these common practices. Our findings reveal that relying on a single neighbor set is suboptimal and that a standard sampling approach can obscure performance trade-offs. Based on this analysis, we propose and validate an initial set of best practices: (1) Incorporation of diverse neighbor sets to balance forget efficacy and model utility, (2) Standard 1:1 sampling methods are inefficient and yield poor results, (3) Our proposed Modular Entity-Level Unlearning (MELU) strategy as an alternative to cyclic sampling. We demonstrate that this modular approach, combined with robust algorithms, provides a clear and stable path towards effective unlearning.

==> ECML_PKDD_2025_Author_Kit/extra.tex <==
\begin{table}[H]
\centering
\caption{Experimental results for different unlearning techniques.}
\label{appendix:unlearning_results}
\begin{tabular}{lccccccc}
\toprule
Method & FE & MU‐R & MU‐T & PPL‐F & PPL‐R & PPL‐T & MMLU \% \\
\midrule
Pre-Unlearning 
  & 0.30  & 0.60  & 0.73  & 38.76 & 37.75 & 37105  & 12.42\\
\midrule
\multicolumn{8}{l}{\textbf{Gradient‐based Unlearning (Untargeted)}} \\
\cmidrule(lr){1-8}
GA                   & 0.44 & 0.54 & 0.67 & 657294.87       & 1551143.40 & 242062.34 & 12.47 \\
Direct          & 0.96  & 0.34  & 0.34  & \(3.09 \times 10^{82}\) & \(8.58 \times 10^{78}\) & \(3.28 \times 10^{80}\) & 13.60\\
Indirect         & 0.89 & 0.59 & 0.65 & \(1.27 \times 10^{90}\) & 8.13 & \(1.79 \times 10^{82}\) & 8.40\\
Balanced        & \(\mathbf{0.97}\)  & 0.48  & 0.55  & \(2.24 \times 10^{85}\) & \(1.75 \times 10^{81}\) & \(1.79 \times 10^{82}\) & 13.29\\
1:1 seq                   & 0.36 & 0.64 & \(\mathbf{0.74}\) & \(3.7 \times 10^{4}\) & 8.36 & \(6.11 \times 10^{4}\) & 12.46 \\
1:1 random & 0.35 & 0.61 & 0.73 & 22521 & 40.01 & 32751 & 12.31 \\
Cyclic          & \(\mathbf{0.97}\)  & 0.57  & 0.65  & \(1.80 \times 10^{86}\) & 3.45             & 3.08 & 13.26 \\
MELU           & 0.89  & 0.61  & 0.70  & \(3.18 \times 10^{90}\) & 6.15 & 15.98  & 13.42\\
\midrule
\multicolumn{8}{l}{\textbf{DPO‐based Unlearning (Targeted)}} \\
\cmidrule(lr){1-8}
DPO                 & 0.70  & 0.31  & 0.47  & 16643 & 2552 & 3098 & 12.21\\
Direct        & 0.57 & 0.78 & 0.76 & \(1.82 \times 10^{4}\) & 2.74 & 158.72 & 12.27\\
Indirect       & 0.71 & 0.80 & 0.77 & \(5.84 \times 10^{7}\) & 2.95 & 180.30 & 12.61 \\
Balanced     & 0.57  & 0.79  & 0.79  & \(1.71 \times 10^{5}\)  & 2.66 & 142.58 & 12.35\\
1:1 seq        & 0.32 & 0.62  & 0.73  & 124.55 & 11.05 & \(3.0 \times 10^{3}\) & 12.33\\
1:1 random & 0.36 & 0.59 & 0.71 & 65.90 & 20.16 & 2539.52 & 12.28 \\
Cyclic        & 0.70  & 0.79  & \textbf{0.80}  & \(2.57 \times 10^{7}\)  & 2.65 & 118.54 & 12.36\\
MELU        & \textbf{0.82} & 0.79 & 0.79 & \(5.8 \times 10^{14}\) & \(2.4 \times 10^{12}\) & 87.71 & 12.38\\
\midrule
\multicolumn{8}{l}{\textbf{NPO‐based Unlearning (Untargeted)}} \\
\cmidrule(lr){1-8}
NPO                 & 0.30  & 0.60  & 0.73  & 38.76 & 37.75 & 37105 & 12.37\\

Direct       & \textbf{0.71} & 0.72 & 0.69 & \(4.68 \times 10^{22}\) & \(2.8 \times 10^{7}\) & \(1.002 \times 10^{17}\) & 12.57\\
Indirect       & 0.60 & 0.78 & 0.78 & \(3.17 \times 10^{18}\) & 4.05 & 126.47 & 12.37 \\
Balanced      & 0.61 & 0.76 & 0.74 & \(2.6 \times 10^{18}\) & 56.04 & 3153.19 & 12.63 \\
1:1 seq        & 0.37 & 0.58 & 0.71 & 1655.97 & 17.42 & \(5.33 \times 10^{5}\) & 12.43\\
1:1 random & 0.35 & 0.60 & 0.72 & 14545.83 & 163.09 & 78544 & 12.36 \\
Cyclic        & 0.63  & 0.77  & 0.78  & \(1.60 \times 10^{18}\) & 6.53 & 35.15 & 12.24\\
MELU         & 0.65 & 0.77 & \textbf{0.79} & \(7.86 \times 10^{21}\) & 3.36 & 54.03 & 12.41\\
\bottomrule
\end{tabular}
\end{table}
